360MonoDepth: High-Resolution 360{\deg} Monocular Depth Estimation

360{\deg} cameras can capture complete environments in a single shot, which makes 360{\deg} imagery alluring in many computer vision tasks. However, monocular depth estimation remains a challenge for 360{\deg} data, particularly for high resolutions like 2K (2048x1024) and beyond that are important for novel-view synthesis and virtual reality applications. Current CNN-based methods do not support such high resolutions due to limited GPU memory. In this work, we propose a flexible framework for monocular depth estimation from high-resolution 360{\deg} images using tangent images. We project the 360{\deg} input image onto a set of tangent planes that produce perspective views, which are suitable for the latest, most accurate state-of-the-art perspective monocular depth estimators. To achieve globally consistent disparity estimates, we recombine the individual depth estimates using deformable multi-scale alignment followed by gradient-domain blending. The result is a dense, high-resolution 360{\deg} depth map with a high level of detail, also for outdoor scenes which are not supported by existing methods. Our source code and data are available at https://manurare.github.io/360monodepth/.

==> figures/quantitative-table-rebuttal.tex <==
\begin{table}[h]
\newcommand{\ul}{\color{blue!70!black}\bf}
\caption{\label{tab:results}%
	Quantitative results for Replica360-4K (new).
	The results shown are using frustum blending (best trade-off between runtime and performance).
	Highlighting: \textbf{best}, {\ul second-best}.%
}
\renewcommand*{\arraystretch}{1.15}%
\setlength{\tabcolsep}{2pt}%
\centering%
\vspace{-0.3cm}
\resizebox{\linewidth}{!}{%
	\begin{tabular}{lccccccc}
		\toprule
		Method & \footnotesize AbsRel \tridown & \footnotesize MAE \tridown & \footnotesize RMSE \tridown & \footnotesize RMSE (log) \tridown & \footnotesize $\delta \!<$1.25 \triup & \footnotesize $\delta \!<$1.25\textsuperscript{2} \triup & \footnotesize $\delta \!<$1.25\textsuperscript{3} \triup \\ \midrule
		OmniDepth                          &     0.337 &     0.582 &     0.778 &     0.161 &     0.484 &     0.785 &     0.920 \\
		BiFuse                             &     0.292 &     0.445 &     0.637 &     0.143 &     0.606 &     0.857 &     0.941 \\
		HoHoNet\MData                      &     0.251 &     0.379 &     0.509 &     0.127 &     0.670 &     0.884 &     0.948 \\
		HoHoNet\SData                      &     0.208 & \ul 0.335 & \bf 0.455 &     0.106 &     0.728 &     0.909 &     0.961 \\
		UniFuse\MData                      &     0.223 & \bf 0.324 & \ul 0.464 &     0.116 &     0.744 &     0.910 &     0.959 \\ \midrule
		Ours\Mvii  (multi-scale)           & \bf 0.150 & \ul 0.335 &     0.558 & \bf 0.081 & \bf 0.813 & \bf 0.953 & \ul 0.983 \\
		Ours\Mviii (multi-scale)           & \ul 0.161 & 	 0.363 &     0.607 & \ul 0.085 & \ul 0.781 & \ul 0.951 & \bf 0.984 \\ \bottomrule
	\end{tabular}%
}\\[1mm]
\footnotesize%
\MData~Trained on Matterport3D %
\qquad\SData~Trained on Stanford 2D-3D-S %
\qquad\Mvii~Using MiDaS v2 %
\qquad\Mviii~Using MiDaS v3 %
\end{table}
